Relation between the Turnaround radius and virial mass in $f(R)$ model

We investigate the relationship between the turnaround radius ($R_t$) and the virial mass ($M_v$) of cosmic structures in the context of $\Lambda$CDM model and in an $f(R)$ model of modified gravity -- namely, the Hu-Sawicki model. The $R_t$ is the distance from the center of the cosmic structure to the shell that is detaching from the Hubble flow at a given time, while the $M_v$ is defined, for this work, as the mass enclosed within the volume where the density is $200$ times the background density. We consider that gravitationally bound astrophysical systems follow a Navarro-Frenk-White density profile, while beyond the virial radius ($R_v$) the profile is approximated by the 2-halo term of the matter correlation function. By combining them together with the information drawn from solving the spherical collapse for the structures, we are able to connect two observables: the $R_t$ and the $M_v$. We show that, in $\Lambda$CDM, the turnaround mass ($M_t$) at $z=0$ is related to the $M_v$ of that same structure by $M_t \simeq 3.07 \, M_v$, while in terms of the radii we have that $R_t \simeq 3.7 \, R_v$ (for $M_v$ of $10^{13} \, h^{-1} \, M_\odot$). In the $f(R)$ model, we have $M_t \simeq 3.43 \, M_v$ and $R_t \simeq 4.1 \, R_v$, for $|f_{R0}|=10^{-6}$ and the same mass scale. Therefore, the difference between $\Lambda$CDM and $f(R)$ in terms of these observable relations is of order $\sim 10-20\%$ even for a relatively mild strength of the modification of gravity ($|f_{R0}|=10^{-6}$). For the $R_t$ itself we find a difference of $\sim 9\%$ between the weakly modification in gravity considered in this work ($|f_{R0}|=10^{-6}$) and $\Lambda$CDM for a mass of $10^{13} \, h^{-1} \, M_\odot$. Once observations allow precisions of this order or better in measurements $R_t$, as well as the $M_v$, these quantities will become powerful tests of modified gravity.

==> bibliografia.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage

\addcontentsline{toc}{chapter}{Referências}

% Referências =====================================================================%
\begin{thebibliography}{12cm}

\bibitem{Riess} Riess, A. G., et al., 2004, ApJ, 607, 655

\bibitem{permutter} S. Perlmutter, et al., 2004, Astrophysics, 607, 655

\bibitem{WessZumino1} Wess, J. and Zumino, B., {\it Nuclear Physics}, {\bf B70}, 39 (1974).

\bibitem{Ryder} Ryder, L. H. {\it Quantum Field Theory}. Cambridge University Press, 1996
(Second Edition).


\bibitem{Grad} Gradshteyn, I. S, Ryzhik, I. M. {\it Table of Integrals, Series and Products: 
Corrected and Enlarged Edition}. Academic Press, Inc. San Diego, 1980.

\end{thebibliography}

%==================================================================================%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

